Capillary driven flows in microgravity

This work investigates the capillary rise dynamics of highly wetting liquids in a divergent U-tube in the microgravity conditions provided by 78th European Space Agency (ESA) parabolic flight. This configuration produces a capillary-driven channel flow. We use image recording in backlight illumination to characterize the interface dynamics and dynamic contact angle of HFE7200 and Di-Propylene Glycol (DPG). For the case of HF7200, we complement the interface measurements with Particle Tracking Velocimetry (PTV) to characterize the velocity fields underneath the moving meniscus. In the experiments with DPG, the liquid column reaches different heights within various experiments, and the measurements show a sharp reduction of the meniscus curvature when the contact line moves from a pre-wet to a dry substrate. In experiments with HFE7200, the interface always moves on a pre-wet surface. Yet a curvature reduction is observed due to the inertial forces on the underlying accelerating flow. The PTV measurements show that the distance from the interface within which the velocity profile adapts to the meniscus velocity shortens as the interface acceleration increases.

==> aps10pt4-1.rtx.tex <==
%%
%% This is file `aps10pt4-1.rtx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% revtex4-1.dtx  (with options: `10pt')
%% 
%% This file is part of the APS files in the REVTeX 4 distribution.
%% For the version number, search on the string 
%% Original version by David Carlisle
%% Modified by Arthur Ogawa (mailto:arthur_ogawa at sbcglobal dot net)
%% 
%% Copyright (c) 2009 The American Physical Society.
%% http://publish.aps.org/revtex4/
%% mailto:revtex4@aps.org
%% 
%% See the REVTeX 4 README file for restrictions and more information.
%% 
\ProvidesFile{aps10pt4-1}
[2010/02/25/18:00:00 4.1p (http://publish.aps.org/revtex4/ for documentation)]% \fileversion
\ifx\undefined\substyle@ext
\def\@tempa{%
	\endinput
	\GenericWarning{I must be read in by REVTeX! (Bailing out)}%
}%
\expandafter\else
\def\@tempa{}%
\expandafter\fi\@tempa
\class@info{RevTeX pointsize 10pt selected}%
\def\normalsize{%
	\@setfontsize\normalsize\@xpt{11.5}%
	\abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip  \abovedisplayskip
	\belowdisplayshortskip \abovedisplayskip
	\let\@listi\@listI
}%
\def\small{%
	\@setfontsize\small\@ixpt{10.5}%
	\abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip \z@ \@plus2\p@
	\belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
	\def\@listi{%
		\leftmargin\leftmargini
		\topsep 4\p@ \@plus2\p@ \@minus2\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep
	}%
}%
\def\footnotesize{%
	\@setfontsize\footnotesize\@viiipt{9.5pt}%
	\abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
	\belowdisplayskip \abovedisplayskip
	\abovedisplayshortskip \z@ \@plus\p@
	\belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
	\def\@listi{%
		\leftmargin\leftmargini
		\topsep 3\p@ \@plus\p@ \@minus\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep
	}%
}%
\def\scriptsize{%
	\@setfontsize\scriptsize\@viipt\@viiipt
}%
\def\tiny{%
	\@setfontsize\tiny\@vpt\@vipt
}%
\def\large{%
	\@setfontsize\large\@xiipt{14pt}%
}%
\def\Large{%
	\@setfontsize\Large\@xivpt{18pt}%
}%
\def\LARGE{%
	\@setfontsize\LARGE\@xviipt{22pt}%
}%
\def\huge{%
	\@setfontsize\huge\@xxpt{25pt}%
}%
\def\Huge{%
	\@setfontsize\Huge\@xxvpt{30pt}%
}%
\appdef\setup@hook{%
	\twoside@sw{%
		\oddsidemargin  -20pt
		\evensidemargin -20pt
		\marginparwidth 107pt
	}{%
		\oddsidemargin  -.25in
		\evensidemargin -.25in
		\marginparwidth 30pt
	}%
}%
\marginparsep 6pt
\topmargin -61pt
\headheight 25pt
\headsep 16pt
\topskip 10pt
\splittopskip\topskip
\footskip 30pt
\textheight = 56pc
\textwidth42.5pc
\columnsep 1.5pc
\columnseprule 0pt
\footnotesep 1pt
\skip\footins 39pt plus 4pt minus 12pt
\def\footnoterule{%
	\dimen@\skip\footins\divide\dimen@\tw@
	\kern-\dimen@\hrule width.5in\kern\dimen@
}%
\floatsep 12pt plus 2pt minus 2pt
\textfloatsep 20pt plus 2pt minus 4pt
\intextsep 12pt plus 2pt minus 2pt
\dblfloatsep 12pt plus 2pt minus 2pt
\dbltextfloatsep 20pt plus 2pt minus 4pt
\@fptop 0pt plus 1fil
\@fpsep 8pt plus 2fil
\@fpbot 0pt plus 1fil
\@dblfptop 0pt plus 1fil
\@dblfpsep 8pt plus 2fil
\@dblfpbot 0pt plus 1fil
\marginparpush 5pt
\parskip 0pt plus 1pt
\parindent 10pt
\emergencystretch8\p@
\partopsep 2pt plus 1pt minus 1pt
\leftmargini 25pt
\leftmarginii 22pt
\leftmarginiii 18.7pt
\leftmarginiv 17pt
\leftmarginv 10pt
\leftmarginvi 10pt
\def\@listI{%
	\leftmargin\leftmargini
	\parsep 4\p@ plus2\p@ minus\p@
	\topsep 8\p@ plus2\p@ minus4\p@
	\itemsep 4\p@ plus2\p@ minus\p@
}%
\labelsep 4pt
\def\@listii{%
	\leftmargin\leftmarginii
	\labelwidth\leftmarginii
	\advance\labelwidth-\labelsep
	\topsep 4\p@ plus2\p@ minus\p@
	\parsep 2\p@ plus\p@ minus\p@
	\itemsep \parsep
}%
\def\@listiii{%
	\leftmargin\leftmarginiii
	\labelwidth\leftmarginiii
	\advance\labelwidth-\labelsep
	\topsep 2\p@ plus\p@ minus\p@
	\parsep \z@
	\partopsep \p@ plus\z@ minus\p@
	\itemsep \topsep
}%
\def\@listiv{%
	\leftmargin\leftmarginiv
	\labelwidth\leftmarginiv
	\advance\labelwidth-\labelsep
}%
\def\@listv{%
	\leftmargin\leftmarginv
	\labelwidth\leftmarginv
	\advance\labelwidth-\labelsep
}%
\def\@listvi{%
	\leftmargin\leftmarginvi
	\labelwidth\leftmarginvi
	\advance\labelwidth-\labelsep
}%
\endinput
%%
%% End of file `aps10pt4-1.rtx'.
